X-ray Selected Galaxy Groups in Bo\"otes

We present the X-ray and optical properties of the galaxy groups selected in the Chandra X-Bo\"otes survey. Our final sample comprises 32 systems at \textbf{$z<1.75$}, with 14 below $z = 0.35$. For these 14 systems we estimate velocity dispersions ($\sigma_{gr}$) and perform a virial analysis to obtain the radii ($R_{200}$ and $R_{500}$) and total masses ($M_{200}$ and $M_{500}$) for groups with at least five galaxy members. We use the Chandra X-ray observations to derive the X-ray luminosity ($L_X$). We examine the performance of the group properties $\sigma_{gr}$, $L_{opt}$ and $L_X$, as proxies for the group mass. Understanding how well these observables measure the total mass is important to estimate how precisely the cluster/group mass function is determined. Exploring the scaling relations built with the X-Bo\"otes sample and comparing these with samples from the literature, we find a break in the $L_X$-$M_{500}$ relation at approximately $M_{500} = 5\times10^{13}$ M$_\odot$ (for $M_{500} > 5\times10^{13}$ M$_\odot$, $M_{500} \propto L_X^{0.61\pm0.02}$, while for $M_{500} \leq 5\times10^{13}$ M$_\odot$, $M_{500} \propto L_X^{0.44\pm0.05}$). Thus, the mass-luminosity relation for galaxy groups cannot be described by the same power law as galaxy clusters. A possible explanation for this break is the dynamical friction, tidal interactions and projection effects which reduce the velocity dispersion values of the galaxy groups. By extending the cluster luminosity function to the group regime, we predict the number of groups that new X-ray surveys, particularly eROSITA, will detect. Based on our cluster/group luminosity function estimates, eROSITA will identify $\sim$1800 groups ($L_X = 10^{41}-10^{43}$ ergs s$^{-1}$) within a distance of 200 Mpc. Since groups lie in large scale filaments, this group sample will map the large scale structure of the local universe.

==> Makefile <==
# Format a latex file as DVI, PS or PDF
LATEX := latex
BIBTEX := bibtex
DVIPS := dvips
PS2PDF := ps2pdf
FORMAT := letter

# Root names for bibtex sources
bibroot := $(basename $(wildcard *.bib))

ALL: bootes_draft.pdf


.SUFFIXES:
.SUFFIXES: .tex .bib .bbl .dvi .ps

.PRECIOUS: %.bbl %.dvi %.ps

# Zap the implicit rule
%.dvi: %.tex


# Pattern rules
%.pdf: %.ps
	$(PS2PDF) $<

%.ps: %.dvi
	$(DVIPS) -Ppdf -G0 -t $(FORMAT) $* -o

%.dvi: %.tex
	while ( \
	  $(LATEX) $* ; \
	  grep -q "Rerun to get \(citations correct\|cross-references right\)" $*.log ) do true ; \
	done

%.bbl: %.tex %.bib
	$(LATEX) $*
	$(BIBTEX) $*


# For latex sources using bibtex
$(addsuffix .dvi,$(bibroot)): %.dvi: %.bbl


clean:
	rm -f *.dvi *.aux *. *.blg *.log *~

vclean: clean
	rm -f *.ps *.bbl

vvclean: vclean
	rm -f *.pdf

